Less is More: Making Smaller Language Models Competent Subgraph Retrievers for Multi-hop KGQA

Retrieval-Augmented Generation (RAG) is widely used to inject external non-parametric knowledge into large language models (LLMs). Recent works suggest that Knowledge Graphs (KGs) contain valuable external knowledge for LLMs. Retrieving information from KGs differs from extracting it from document sets. Most existing approaches seek to directly retrieve relevant subgraphs, thereby eliminating the need for extensive SPARQL annotations, traditionally required by semantic parsing methods. In this paper, we model the subgraph retrieval task as a conditional generation task handled by small language models. Specifically, we define a subgraph identifier as a sequence of relations, each represented as a special token stored in the language models. Our base generative subgraph retrieval model, consisting of only 220M parameters, achieves competitive retrieval performance compared to state-of-the-art models relying on 7B parameters, demonstrating that small language models are capable of performing the subgraph retrieval task. Furthermore, our largest 3B model, when plugged with an LLM reader, sets new SOTA end-to-end performance on both the WebQSP and CWQ benchmarks. Our model and data will be made available online: https://github.com/hwy9855/GSR.

==> tables/detailed_results.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l|ccc|ccc}
    \toprule
        \multirow{2}{*}{\bf{Model}} & \multicolumn{3}{c}{\bf{WebQSP}} & \multicolumn{3}{|c}{\bf{CWQ}} \\ 
        & P & R & F1 & P & R & F1 \\ \midrule
        \multicolumn{7}{c}{\it{Dual Encoder based subgraph retrieval}} \\ 
        \midrule
        SR & \\ \midrule
        \multicolumn{7}{c}{\it{LLM based subgraph retrieval}} \\ \midrule 
        RoG & 46.90 & 79.85 & 49.56 & 18.88 & 67.89 & 22.26 \\
        \midrule
        \multicolumn{7}{c}{\it{ours w/ raw data}} \\ \midrule
        GSR-base & 42.17 & 84.38 & 47.02 & 17.70 & 72.57 & 21.61 \\
        GSR-large & 46.84 & 86.69 & 49.41 & 19.21 & 73.78 & 22.54 \\
        GSR-3b & 46.92 & 86.54 & 49.65 & 19.72 & 73.46 & 23.07 \\ \midrule 
        \multicolumn{7}{c}{\it{ours w/ filtered data}} \\ \midrule
        GSR-base & 47.90 & 85.35 & 53.87 & 21.43 & 72.33 & 26.09\\
        GSR-large & 49.48 & 86.80 & 53.87 & 21.45 & 73.88 & 26.15\\
        GSR-3b & 50.45 & 87.51 & 55.36 & 21.64 & 73.70 & 26.43 \\ 
        \midrule
        \multicolumn{7}{c}{\it{ours w/ gpt selected data}} \\ \midrule
        GSR-base & 52.75 & 84.31 & 57.41 & 21.69 & 71.96 & 26.33\\
        GSR-large & 56.25 & 85.90 & 58.69 & 23.98 & 73.17 & 27.71 \\
        GSR-3b & 58.84 & 86.50 & 60.58 & 24.08 & 73.38 & 28.05\\
        \bottomrule
    \end{tabular}
    \caption{Subgraph Retrieval Results. Our GSR model is first pretrained on indexing data (pseudo question), and then finetuned on weakly supervised data with different settings.}
    \label{tab:}
\end{table*}

